Upper limits on gravitational wave emission from 78 radio pulsars

We present upper limits on the gravitational wave emission from 78 radio pulsars based on data from the third and fourth science runs of the LIGO and GEO600 gravitational wave detectors. The data from both runs have been combined coherently to maximise sensitivity. For the first time pulsars within binary (or multiple) systems have been included in the search by taking into account the signal modulation due to their orbits. Our upper limits are therefore the first measured for 56 of these pulsars. For the remaining 22, our results improve on previous upper limits by up to a factor of 10. For example, our tightest upper limit on the gravitational strain is 2.6e-25 for PSRJ1603-7202, and the equatorial ellipticity of PSRJ2124-3358 is less than 10^{-6}. Furthermore, our strain upper limit for the Crab pulsar is only 2.2 times greater than the fiducial spin-down limit.

==> authorlist.tex <==
\makeatletter
\def\@fnsymbol#1{\ifcase#1\or * \or  $+$ \or  \$ \or \#  \or \dag \or \ddag \or
$\mathsection$ \or $ \mathparagraph$ \or $\|$  \or
\textordfeminine \or \textbullet   \or ** \or $++$ \or  \$\$ \or
\#\#  \or \dag\dag \or \ddag\ddag \or $\mathsection\mathsection$
\or $ \mathparagraph\mathparagraph$ \or $\|\|$  \or
\textordfeminine\textordfeminine \or \textbullet \textbullet \or
*** \or $+++$ \or  \$\$\$ \or \#\#  \or \dag\dag \or \ddag\ddag
\or $\mathsection \mathsection\mathsection$ \or $ \mathparagraph
\mathparagraph\mathparagraph$ \or $\|\|\|$  \or
\textordfeminine\textordfeminine\textordfeminine \or
\textbullet\textbullet\textbullet \or \else \@ctrerr\fi}

\makeatother

\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur Gravitationsphysik, D-14476 Golm,
Germany}
\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur Gravitationsphysik, D-30167
Hannover, Germany}
\affiliation{Andrews University, Berrien Springs, MI 49104 USA}
\affiliation{Australian National University, Canberra, 0200, Australia}
\affiliation{California Institute of Technology, Pasadena, CA  91125, USA}
\affiliation{California State University Dominguez Hills, Carson, CA  90747, USA}
\affiliation{Caltech-CaRT, Pasadena, CA  91125, USA}
\affiliation{Cardiff University, Cardiff, CF2 3YB, United Kingdom}
\affiliation{Carleton College, Northfield, MN  55057, USA}
\affiliation{Charles Sturt University, Wagga Wagga, NSW 2678, Australia}
\affiliation{Columbia University, New York, NY  10027, USA}
\affiliation{Embry-Riddle Aeronautical University, Prescott, AZ   86301 USA}
\affiliation{Hobart and William Smith Colleges, Geneva, NY  14456, USA}
\affiliation{Inter-University Centre for Astronomy  and Astrophysics, Pune - 411007, India}
\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\affiliation{LIGO Hanford Observatory, Richland, WA  99352, USA}
\affiliation{LIGO Livingston Observatory, Livingston, LA  70754, USA}
\affiliation{LIGO - Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\affiliation{Louisiana State University, Baton Rouge, LA  70803, USA}
\affiliation{Louisiana Tech University, Ruston, LA  71272, USA}
\affiliation{Loyola University, New Orleans, LA 70118, USA}
\affiliation{Moscow State University, Moscow, 119992, Russia}
\affiliation{NASA/Goddard Space Flight Center, Greenbelt, MD  20771, USA}
\affiliation{National Astronomical Observatory of Japan, Tokyo  181-8588, Japan}
\affiliation{Northwestern University, Evanston, IL  60208, USA}
\affiliation{Rochester Institute of Technology, Rochester, NY 14623, USA}
\affiliation{Rutherford Appleton Laboratory, Chilton, Didcot, Oxon OX11 0QX United Kingdom}
\affiliation{San Jose State University, San Jose, CA 95192, USA}
\affiliation{Southeastern Louisiana University, Hammond, LA  70402, USA}
\affiliation{Southern University and A\&M College, Baton Rouge, LA  70813, USA}
\affiliation{Stanford University, Stanford, CA  94305, USA}
\affiliation{Syracuse University, Syracuse, NY  13244, USA}
\affiliation{The Pennsylvania State University, University Park, PA  16802, USA}
\affiliation{The University of Texas at Brownsville and Texas Southmost College, Brownsville, TX 
78520, USA}
\affiliation{Trinity University, San Antonio, TX  78212, USA}
\affiliation{Universitat de les Illes Balears, E-07122 Palma de Mallorca, Spain}
\affiliation{Universit\"at Hannover, D-30167 Hannover, Germany}
\affiliation{University of Adelaide, Adelaide, SA 5005, Australia}
\affiliation{University of Birmingham, Birmingham, B15 2TT, United Kingdom}
\affiliation{University of Florida, Gainesville, FL  32611, USA}
\affiliation{University of Glasgow, Glasgow, G12 8QQ, United Kingdom}
\affiliation{University of Maryland, College Park, MD 20742 USA}
\affiliation{University of Michigan, Ann Arbor, MI  48109, USA}
\affiliation{University of Oregon, Eugene, OR  97403, USA}
\affiliation{University of Rochester, Rochester, NY  14627, USA}
\affiliation{University of Salerno, 84084 Fisciano (Salerno), Italy}
\affiliation{University of Sannio at Benevento, I-82100 Benevento, Italy}
\affiliation{University of Southampton, Southampton, SO17 1BJ, United Kingdom}
\affiliation{University of Strathclyde, Glasgow, G1 1XQ, United Kingdom}
\affiliation{University of Washington, Seattle, WA, 98195}
\affiliation{University of Western Australia, Crawley, WA 6009, Australia}
\affiliation{University of Wisconsin-Milwaukee, Milwaukee, WI  53201, USA}
\affiliation{Vassar College, Poughkeepsie, NY 12604}
\affiliation{Washington State University, Pullman, WA 99164, USA}
\affiliation{University of Manchester, Jodrell Bank Observatory, Macclesfield, SK11 9DL, United
Kingdom}
\author{B.~Abbott}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{R.~Abbott}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{R.~Adhikari}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125,
USA}
\author{J.~Agresti}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{P.~Ajith}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur
Gravitationsphysik, D-30167 Hannover, Germany}
\author{B.~Allen}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur
Gravitationsphysik, D-30167 Hannover, Germany}\affiliation{University of Wisconsin-Milwaukee,
Milwaukee, WI  53201, USA}
\author{R.~Amin}\affiliation{Louisiana State University, Baton Rouge, LA  70803, USA}
\author{S.~B.~Anderson}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125,
USA}
\author{W.~G.~Anderson}\affiliation{University of Wisconsin-Milwaukee, Milwaukee, WI  53201, USA}
\author{M.~Arain}\affiliation{University of Florida, Gainesville, FL  32611, USA}
\author{M.~Araya}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{H.~Armandula}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125,
USA}
\author{M.~Ashley}\affiliation{Australian National University, Canberra, 0200, Australia}
\author{S.~Aston}\affiliation{University of Birmingham, Birmingham, B15 2TT, United Kingdom}
\author{P.~Aufmuth}\affiliation{Universit\"at Hannover, D-30167 Hannover, Germany}
\author{C.~Aulbert}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur
Gravitationsphysik, D-14476 Golm, Germany}
\author{S.~Babak}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur
Gravitationsphysik, D-14476 Golm, Germany}
\author{S.~Ballmer}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{H.~Bantilan}\affiliation{Carleton College, Northfield, MN  55057, USA}
\author{B.~C.~Barish}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125,
USA}
\author{C.~Barker}\affiliation{LIGO Hanford Observatory, Richland, WA  99352, USA}
\author{D.~Barker}\affiliation{LIGO Hanford Observatory, Richland, WA  99352, USA}
\author{B.~Barr}\affiliation{University of Glasgow, Glasgow, G12 8QQ, United Kingdom}
\author{P.~Barriga}\affiliation{University of Western Australia, Crawley, WA 6009, Australia}
\author{M.~A.~Barton}\affiliation{University of Glasgow, Glasgow, G12 8QQ, United Kingdom}
\author{K.~Bayer}\affiliation{LIGO - Massachusetts Institute of Technology, Cambridge, MA 02139,
USA}
\author{K.~Belczynski}\affiliation{Northwestern University, Evanston, IL  60208, USA}
\author{J.~Betzwieser}\affiliation{LIGO - Massachusetts Institute of Technology, Cambridge, MA
02139, USA}
\author{P.~T.~Beyersdorf}\affiliation{San Jose State University, San Jose, CA 95192, USA}
\author{B.~Bhawal}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{I.~A.~Bilenko}\affiliation{Moscow State University, Moscow, 119992, Russia}
\author{G.~Billingsley}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125,
USA}
\author{R.~Biswas}\affiliation{University of Wisconsin-Milwaukee, Milwaukee, WI  53201, USA}
\author{E.~Black}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{K.~Blackburn}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125,
USA}
\author{L.~Blackburn}\affiliation{LIGO - Massachusetts Institute of Technology, Cambridge, MA 02139,
USA}
\author{D.~Blair}\affiliation{University of Western Australia, Crawley, WA 6009, Australia}
\author{B.~Bland}\affiliation{LIGO Hanford Observatory, Richland, WA  99352, USA}
\author{J.~Bogenstahl}\affiliation{University of Glasgow, Glasgow, G12 8QQ, United Kingdom}
\author{L.~Bogue}\affiliation{LIGO Livingston Observatory, Livingston, LA  70754, USA}
\author{R.~Bork}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{V.~Boschi}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{S.~Bose}\affiliation{Washington State University, Pullman, WA 99164, USA}
\author{P.~R.~Brady}\affiliation{University of Wisconsin-Milwaukee, Milwaukee, WI  53201, USA}
\author{V.~B.~Braginsky}\affiliation{Moscow State University, Moscow, 119992, Russia}
\author{J.~E.~Brau}\affiliation{University of Oregon, Eugene, OR  97403, USA}
\author{M.~Brinkmann}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur
Gravitationsphysik, D-30167 Hannover, Germany}
\author{A.~Brooks}\affiliation{University of Adelaide, Adelaide, SA 5005, Australia}
\author{D.~A.~Brown}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125,
USA}\affiliation{Caltech-CaRT, Pasadena, CA  91125, USA}
\author{A.~Bullington}\affiliation{Stanford University, Stanford, CA  94305, USA}
\author{A.~Bunkowski}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur
Gravitationsphysik, D-30167 Hannover, Germany}
\author{A.~Buonanno}\affiliation{University of Maryland, College Park, MD 20742 USA}
\author{O.~Burmeister}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur
Gravitationsphysik, D-30167 Hannover, Germany}
\author{D.~Busby}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{W.~E.~Butler}\affiliation{University of Rochester, Rochester, NY  14627, USA}
\author{R.~L.~Byer}\affiliation{Stanford University, Stanford, CA  94305, USA}
\author{L.~Cadonati}\affiliation{LIGO - Massachusetts Institute of Technology, Cambridge, MA 02139,
USA}
\author{G.~Cagnoli}\affiliation{University of Glasgow, Glasgow, G12 8QQ, United Kingdom}
\author{J.~B.~Camp}\affiliation{NASA/Goddard Space Flight Center, Greenbelt, MD  20771, USA}
\author{J.~Cannizzo}\affiliation{NASA/Goddard Space Flight Center, Greenbelt, MD  20771, USA}
\author{K.~Cannon}\affiliation{University of Wisconsin-Milwaukee, Milwaukee, WI  53201, USA}
\author{C.~A.~Cantley}\affiliation{University of Glasgow, Glasgow, G12 8QQ, United Kingdom}
\author{J.~Cao}\affiliation{LIGO - Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{L.~Cardenas}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125,
USA}
\author{K.~Carter}\affiliation{LIGO Livingston Observatory, Livingston, LA  70754, USA}
\author{M.~M.~Casey}\affiliation{University of Glasgow, Glasgow, G12 8QQ, United Kingdom}
\author{G.~Castaldi}\affiliation{University of Sannio at Benevento, I-82100 Benevento, Italy}
\author{C.~Cepeda}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{E.~Chalkey}\affiliation{University of Glasgow, Glasgow, G12 8QQ, United Kingdom}
\author{P.~Charlton}\affiliation{Charles Sturt University, Wagga Wagga, NSW 2678, Australia}
\author{S.~Chatterji}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125,
USA}
\author{S.~Chelkowski}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur
Gravitationsphysik, D-30167 Hannover, Germany}
\author{Y.~Chen}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur Gravitationsphysik,
D-14476 Golm, Germany}
\author{F.~Chiadini}\affiliation{University of Salerno, 84084 Fisciano (Salerno), Italy}
\author{D.~Chin}\affiliation{University of Michigan, Ann Arbor, MI  48109, USA}
\author{E.~Chin}\affiliation{University of Western Australia, Crawley, WA 6009, Australia}
\author{J.~Chow}\affiliation{Australian National University, Canberra, 0200, Australia}
\author{N.~Christensen}\affiliation{Carleton College, Northfield, MN  55057, USA}
\author{J.~Clark}\affiliation{University of Glasgow, Glasgow, G12 8QQ, United Kingdom}
\author{P.~Cochrane}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur
Gravitationsphysik, D-30167 Hannover, Germany}
\author{T.~Cokelaer}\affiliation{Cardiff University, Cardiff, CF2 3YB, United Kingdom}
\author{C.~N.~Colacino}\affiliation{University of Birmingham, Birmingham, B15 2TT, United Kingdom}
\author{R.~Coldwell}\affiliation{University of Florida, Gainesville, FL  32611, USA}
\author{R.~Conte}\affiliation{University of Salerno, 84084 Fisciano (Salerno), Italy}
\author{D.~Cook}\affiliation{LIGO Hanford Observatory, Richland, WA  99352, USA}
\author{T.~Corbitt}\affiliation{LIGO - Massachusetts Institute of Technology, Cambridge, MA 02139,
USA}
\author{D.~Coward}\affiliation{University of Western Australia, Crawley, WA 6009, Australia}
\author{D.~Coyne}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{J.~D.~E.~Creighton}\affiliation{University of Wisconsin-Milwaukee, Milwaukee, WI  53201,
USA}
\author{T.~D.~Creighton}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125,
USA}
\author{R.~P.~Croce}\affiliation{University of Sannio at Benevento, I-82100 Benevento, Italy}
\author{D.~R.~M.~Crooks}\affiliation{University of Glasgow, Glasgow, G12 8QQ, United Kingdom}
\author{A.~M.~Cruise}\affiliation{University of Birmingham, Birmingham, B15 2TT, United Kingdom}
\author{A.~Cumming}\affiliation{University of Glasgow, Glasgow, G12 8QQ, United Kingdom}
\author{J.~Dalrymple}\affiliation{Syracuse University, Syracuse, NY  13244, USA}
\author{E.~D'Ambrosio}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125,
USA}
\author{K.~Danzmann}\affiliation{Universit\"at Hannover, D-30167 Hannover,
Germany}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur Gravitationsphysik, D-30167
Hannover, Germany}
\author{G.~Davies}\affiliation{Cardiff University, Cardiff, CF2 3YB, United Kingdom}
\author{D.~DeBra}\affiliation{Stanford University, Stanford, CA  94305, USA}
\author{J.~Degallaix}\affiliation{University of Western Australia, Crawley, WA 6009, Australia}
\author{M.~Degree}\affiliation{Stanford University, Stanford, CA  94305, USA}
\author{T.~Demma}\affiliation{University of Sannio at Benevento, I-82100 Benevento, Italy}
\author{V.~Dergachev}\affiliation{University of Michigan, Ann Arbor, MI  48109, USA}
\author{S.~Desai}\affiliation{The Pennsylvania State University, University Park, PA  16802, USA}
\author{R.~DeSalvo}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{S.~Dhurandhar}\affiliation{Inter-University Centre for Astronomy  and Astrophysics, Pune -
411007, India}
\author{M.~D\'iaz}\affiliation{The University of Texas at Brownsville and Texas Southmost College,
Brownsville, TX  78520, USA}
\author{J.~Dickson}\affiliation{Australian National University, Canberra, 0200, Australia}
\author{A.~Di~Credico}\affiliation{Syracuse University, Syracuse, NY  13244, USA}
\author{G.~Diederichs}\affiliation{Universit\"at Hannover, D-30167 Hannover, Germany}
\author{A.~Dietz}\affiliation{Cardiff University, Cardiff, CF2 3YB, United Kingdom}
\author{E.~E.~Doomes}\affiliation{Southern University and A\&M College, Baton Rouge, LA  70813, USA}
\author{R.~W.~P.~Drever}\affiliation{California Institute of Technology, Pasadena, CA  91125, USA}
\author{J.-C.~Dumas}\affiliation{University of Western Australia, Crawley, WA 6009, Australia}
\author{R.~J.~Dupuis}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125,
USA}
\author{J.~G.~Dwyer}\affiliation{Columbia University, New York, NY  10027, USA}
\author{P.~Ehrens}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{E.~Espinoza}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125,
USA}
\author{T.~Etzel}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{M.~Evans}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{T.~Evans}\affiliation{LIGO Livingston Observatory, Livingston, LA  70754, USA}
\author{S.~Fairhurst}\affiliation{Cardiff University, Cardiff, CF2 3YB, United
Kingdom}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{Y.~Fan}\affiliation{University of Western Australia, Crawley, WA 6009, Australia}
\author{D.~Fazi}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{M.~M.~Fejer}\affiliation{Stanford University, Stanford, CA  94305, USA}
\author{L.~S.~Finn}\affiliation{The Pennsylvania State University, University Park, PA  16802, USA}
\author{V.~Fiumara}\affiliation{University of Salerno, 84084 Fisciano (Salerno), Italy}
\author{N.~Fotopoulos}\affiliation{University of Wisconsin-Milwaukee, Milwaukee, WI  53201, USA}
\author{A.~Franzen}\affiliation{Universit\"at Hannover, D-30167 Hannover, Germany}
\author{K.~Y.~Franzen}\affiliation{University of Florida, Gainesville, FL  32611, USA}
\author{A.~Freise}\affiliation{University of Birmingham, Birmingham, B15 2TT, United Kingdom}
\author{R.~Frey}\affiliation{University of Oregon, Eugene, OR  97403, USA}
\author{T.~Fricke}\affiliation{University of Rochester, Rochester, NY  14627, USA}
\author{P.~Fritschel}\affiliation{LIGO - Massachusetts Institute of Technology, Cambridge, MA 02139,
USA}
\author{V.~V.~Frolov}\affiliation{LIGO Livingston Observatory, Livingston, LA  70754, USA}
\author{M.~Fyffe}\affiliation{LIGO Livingston Observatory, Livingston, LA  70754, USA}
\author{V.~Galdi}\affiliation{University of Sannio at Benevento, I-82100 Benevento, Italy}
\author{K.~S.~Ganezer}\affiliation{California State University Dominguez Hills, Carson, CA  90747,
USA}
\author{J.~Garofoli}\affiliation{LIGO Hanford Observatory, Richland, WA  99352, USA}
\author{I.~Gholami}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur
Gravitationsphysik, D-14476 Golm, Germany}
\author{J.~A.~Giaime}\affiliation{LIGO Livingston Observatory, Livingston, LA  70754,
USA}\affiliation{Louisiana State University, Baton Rouge, LA  70803, USA}
\author{S.~Giampanis}\affiliation{University of Rochester, Rochester, NY  14627, USA}
\author{K.~D.~Giardina}\affiliation{LIGO Livingston Observatory, Livingston, LA  70754, USA}
\author{K.~Goda}\affiliation{LIGO - Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{E.~Goetz}\affiliation{University of Michigan, Ann Arbor, MI  48109, USA}
\author{L.~Goggin}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{G.~Gonz\'alez}\affiliation{Louisiana State University, Baton Rouge, LA  70803, USA}
\author{S.~Gossler}\affiliation{Australian National University, Canberra, 0200, Australia}
\author{A.~Grant}\affiliation{University of Glasgow, Glasgow, G12 8QQ, United Kingdom}
\author{S.~Gras}\affiliation{University of Western Australia, Crawley, WA 6009, Australia}
\author{C.~Gray}\affiliation{LIGO Hanford Observatory, Richland, WA  99352, USA}
\author{M.~Gray}\affiliation{Australian National University, Canberra, 0200, Australia}
\author{J.~Greenhalgh}\affiliation{Rutherford Appleton Laboratory, Chilton, Didcot, Oxon OX11 0QX
United Kingdom}
\author{A.~M.~Gretarsson}\affiliation{Embry-Riddle Aeronautical University, Prescott, AZ   86301
USA}
\author{R.~Grosso}\affiliation{The University of Texas at Brownsville and Texas Southmost College,
Brownsville, TX  78520, USA}
\author{H.~Grote}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur
Gravitationsphysik, D-30167 Hannover, Germany}
\author{S.~Grunewald}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur
Gravitationsphysik, D-14476 Golm, Germany}
\author{M.~Guenther}\affiliation{LIGO Hanford Observatory, Richland, WA  99352, USA}
\author{R.~Gustafson}\affiliation{University of Michigan, Ann Arbor, MI  48109, USA}
\author{B.~Hage}\affiliation{Universit\"at Hannover, D-30167 Hannover, Germany}
\author{D.~Hammer}\affiliation{University of Wisconsin-Milwaukee, Milwaukee, WI  53201, USA}
\author{C.~Hanna}\affiliation{Louisiana State University, Baton Rouge, LA  70803, USA}
\author{J.~Hanson}\affiliation{LIGO Livingston Observatory, Livingston, LA  70754, USA}
\author{J.~Harms}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur
Gravitationsphysik, D-30167 Hannover, Germany}
\author{G.~Harry}\affiliation{LIGO - Massachusetts Institute of Technology, Cambridge, MA 02139,
USA}
\author{E.~Harstad}\affiliation{University of Oregon, Eugene, OR  97403, USA}
\author{T.~Hayler}\affiliation{Rutherford Appleton Laboratory, Chilton, Didcot, Oxon OX11 0QX United
Kingdom}
\author{J.~Heefner}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{I.~S.~Heng}\affiliation{University of Glasgow, Glasgow, G12 8QQ, United Kingdom}
\author{A.~Heptonstall}\affiliation{University of Glasgow, Glasgow, G12 8QQ, United Kingdom}
\author{M.~Heurs}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur
Gravitationsphysik, D-30167 Hannover, Germany}
\author{M.~Hewitson}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur
Gravitationsphysik, D-30167 Hannover, Germany}
\author{S.~Hild}\affiliation{Universit\"at Hannover, D-30167 Hannover, Germany}
\author{E.~Hirose}\affiliation{Syracuse University, Syracuse, NY  13244, USA}
\author{D.~Hoak}\affiliation{LIGO Livingston Observatory, Livingston, LA  70754, USA}
\author{D.~Hosken}\affiliation{University of Adelaide, Adelaide, SA 5005, Australia}
\author{J.~Hough}\affiliation{University of Glasgow, Glasgow, G12 8QQ, United Kingdom}
\author{E.~Howell}\affiliation{University of Western Australia, Crawley, WA 6009, Australia}
\author{D.~Hoyland}\affiliation{University of Birmingham, Birmingham, B15 2TT, United Kingdom}
\author{S.~H.~Huttner}\affiliation{University of Glasgow, Glasgow, G12 8QQ, United Kingdom}
\author{D.~Ingram}\affiliation{LIGO Hanford Observatory, Richland, WA  99352, USA}
\author{E.~Innerhofer}\affiliation{LIGO - Massachusetts Institute of Technology, Cambridge, MA
02139, USA}
\author{M.~Ito}\affiliation{University of Oregon, Eugene, OR  97403, USA}
\author{Y.~Itoh}\affiliation{University of Wisconsin-Milwaukee, Milwaukee, WI  53201, USA}
\author{A.~Ivanov}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{D.~Jackrel}\affiliation{Stanford University, Stanford, CA  94305, USA}
\author{B.~Johnson}\affiliation{LIGO Hanford Observatory, Richland, WA  99352, USA}
\author{W.~W.~Johnson}\affiliation{Louisiana State University, Baton Rouge, LA  70803, USA}
\author{D.~I.~Jones}\affiliation{University of Southampton, Southampton, SO17 1BJ, United Kingdom}
\author{G.~Jones}\affiliation{Cardiff University, Cardiff, CF2 3YB, United Kingdom}
\author{R.~Jones}\affiliation{University of Glasgow, Glasgow, G12 8QQ, United Kingdom}
\author{L.~Ju}\affiliation{University of Western Australia, Crawley, WA 6009, Australia}
\author{P.~Kalmus}\affiliation{Columbia University, New York, NY  10027, USA}
\author{V.~Kalogera}\affiliation{Northwestern University, Evanston, IL  60208, USA}
\author{D.~Kasprzyk}\affiliation{University of Birmingham, Birmingham, B15 2TT, United Kingdom}
\author{E.~Katsavounidis}\affiliation{LIGO - Massachusetts Institute of Technology, Cambridge, MA
02139, USA}
\author{K.~Kawabe}\affiliation{LIGO Hanford Observatory, Richland, WA  99352, USA}
\author{S.~Kawamura}\affiliation{National Astronomical Observatory of Japan, Tokyo  181-8588, Japan}
\author{F.~Kawazoe}\affiliation{National Astronomical Observatory of Japan, Tokyo  181-8588, Japan}
\author{W.~Kells}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{D.~G.~Keppel}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125,
USA}
\author{F.~Ya.~Khalili}\affiliation{Moscow State University, Moscow, 119992, Russia}
\author{C.~Kim}\affiliation{Northwestern University, Evanston, IL  60208, USA}
\author{P.~King}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{J.~S.~Kissel}\affiliation{Louisiana State University, Baton Rouge, LA  70803, USA}
\author{S.~Klimenko}\affiliation{University of Florida, Gainesville, FL  32611, USA}
\author{K.~Kokeyama}\affiliation{National Astronomical Observatory of Japan, Tokyo  181-8588, Japan}
\author{V.~Kondrashov}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125,
USA}
\author{R.~K.~Kopparapu}\affiliation{Louisiana State University, Baton Rouge, LA  70803, USA}
\author{D.~Kozak}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{B.~Krishnan}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur
Gravitationsphysik, D-14476 Golm, Germany}
\author{P.~Kwee}\affiliation{Universit\"at Hannover, D-30167 Hannover, Germany}
\author{P.~K.~Lam}\affiliation{Australian National University, Canberra, 0200, Australia}
\author{M.~Landry}\affiliation{LIGO Hanford Observatory, Richland, WA  99352, USA}
\author{B.~Lantz}\affiliation{Stanford University, Stanford, CA  94305, USA}
\author{A.~Lazzarini}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125,
USA}
\author{B.~Lee}\affiliation{University of Western Australia, Crawley, WA 6009, Australia}
\author{M.~Lei}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{J.~Leiner}\affiliation{Washington State University, Pullman, WA 99164, USA}
\author{V.~Leonhardt}\affiliation{National Astronomical Observatory of Japan, Tokyo  181-8588,
Japan}
\author{I.~Leonor}\affiliation{University of Oregon, Eugene, OR  97403, USA}
\author{K.~Libbrecht}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125,
USA}
\author{P.~Lindquist}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125,
USA}
\author{N.~A.~Lockerbie}\affiliation{University of Strathclyde, Glasgow, G1 1XQ, United Kingdom}
\author{M.~Longo}\affiliation{University of Salerno, 84084 Fisciano (Salerno), Italy}
\author{M.~Lormand}\affiliation{LIGO Livingston Observatory, Livingston, LA  70754, USA}
\author{M.~Lubinski}\affiliation{LIGO Hanford Observatory, Richland, WA  99352, USA}
\author{H.~L\"uck}\affiliation{Universit\"at Hannover, D-30167 Hannover,
Germany}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur Gravitationsphysik, D-30167
Hannover, Germany}
\author{B.~Machenschalk}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur
Gravitationsphysik, D-14476 Golm, Germany}
\author{M.~MacInnis}\affiliation{LIGO - Massachusetts Institute of Technology, Cambridge, MA 02139,
USA}
\author{M.~Mageswaran}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125,
USA}
\author{K.~Mailand}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{M.~Malec}\affiliation{Universit\"at Hannover, D-30167 Hannover, Germany}
\author{V.~Mandic}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{S.~Marano}\affiliation{University of Salerno, 84084 Fisciano (Salerno), Italy}
\author{S.~M\'arka}\affiliation{Columbia University, New York, NY  10027, USA}
\author{J.~Markowitz}\affiliation{LIGO - Massachusetts Institute of Technology, Cambridge, MA 02139,
USA}
\author{E.~Maros}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{I.~Martin}\affiliation{University of Glasgow, Glasgow, G12 8QQ, United Kingdom}
\author{J.~N.~Marx}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{K.~Mason}\affiliation{LIGO - Massachusetts Institute of Technology, Cambridge, MA 02139,
USA}
\author{L.~Matone}\affiliation{Columbia University, New York, NY  10027, USA}
\author{V.~Matta}\affiliation{University of Salerno, 84084 Fisciano (Salerno), Italy}
\author{N.~Mavalvala}\affiliation{LIGO - Massachusetts Institute of Technology, Cambridge, MA 02139,
USA}
\author{R.~McCarthy}\affiliation{LIGO Hanford Observatory, Richland, WA  99352, USA}
\author{D.~E.~McClelland}\affiliation{Australian National University, Canberra, 0200, Australia}
\author{S.~C.~McGuire}\affiliation{Southern University and A\&M College, Baton Rouge, LA  70813,
USA}
\author{M.~McHugh}\affiliation{Loyola University, New Orleans, LA 70118, USA}
\author{K.~McKenzie}\affiliation{Australian National University, Canberra, 0200, Australia}
\author{J.~W.~C.~McNabb}\affiliation{The Pennsylvania State University, University Park, PA  16802,
USA}
\author{S.~McWilliams}\affiliation{NASA/Goddard Space Flight Center, Greenbelt, MD  20771, USA}
\author{T.~Meier}\affiliation{Universit\"at Hannover, D-30167 Hannover, Germany}
\author{A.~Melissinos}\affiliation{University of Rochester, Rochester, NY  14627, USA}
\author{G.~Mendell}\affiliation{LIGO Hanford Observatory, Richland, WA  99352, USA}
\author{R.~A.~Mercer}\affiliation{University of Florida, Gainesville, FL  32611, USA}
\author{S.~Meshkov}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{E.~Messaritaki}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125,
USA}
\author{C.~J.~Messenger}\affiliation{University of Glasgow, Glasgow, G12 8QQ, United Kingdom}
\author{D.~Meyers}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{E.~Mikhailov}\affiliation{LIGO - Massachusetts Institute of Technology, Cambridge, MA 02139,
USA}
\author{S.~Mitra}\affiliation{Inter-University Centre for Astronomy  and Astrophysics, Pune -
411007, India}
\author{V.~P.~Mitrofanov}\affiliation{Moscow State University, Moscow, 119992, Russia}
\author{G.~Mitselmakher}\affiliation{University of Florida, Gainesville, FL  32611, USA}
\author{R.~Mittleman}\affiliation{LIGO - Massachusetts Institute of Technology, Cambridge, MA 02139,
USA}
\author{O.~Miyakawa}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125,
USA}
\author{S.~Mohanty}\affiliation{The University of Texas at Brownsville and Texas Southmost College,
Brownsville, TX  78520, USA}
\author{G.~Moreno}\affiliation{LIGO Hanford Observatory, Richland, WA  99352, USA}
\author{K.~Mossavi}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur
Gravitationsphysik, D-30167 Hannover, Germany}
\author{C.~MowLowry}\affiliation{Australian National University, Canberra, 0200, Australia}
\author{A.~Moylan}\affiliation{Australian National University, Canberra, 0200, Australia}
\author{D.~Mudge}\affiliation{University of Adelaide, Adelaide, SA 5005, Australia}
\author{G.~Mueller}\affiliation{University of Florida, Gainesville, FL  32611, USA}
\author{S.~Mukherjee}\affiliation{The University of Texas at Brownsville and Texas Southmost
College, Brownsville, TX  78520, USA}
\author{H.~M\"uller-Ebhardt}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur
Gravitationsphysik, D-30167 Hannover, Germany}
\author{J.~Munch}\affiliation{University of Adelaide, Adelaide, SA 5005, Australia}
\author{P.~Murray}\affiliation{University of Glasgow, Glasgow, G12 8QQ, United Kingdom}
\author{E.~Myers}\affiliation{LIGO Hanford Observatory, Richland, WA  99352, USA}
\author{J.~Myers}\affiliation{LIGO Hanford Observatory, Richland, WA  99352, USA}
\author{T.~Nash}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{G.~Newton}\affiliation{University of Glasgow, Glasgow, G12 8QQ, United Kingdom}
\author{A.~Nishizawa}\affiliation{National Astronomical Observatory of Japan, Tokyo  181-8588,
Japan}
\author{F.~Nocera}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{K.~Numata}\affiliation{NASA/Goddard Space Flight Center, Greenbelt, MD  20771, USA}
\author{B.~O'Reilly}\affiliation{LIGO Livingston Observatory, Livingston, LA  70754, USA}
\author{R.~O'Shaughnessy}\affiliation{Northwestern University, Evanston, IL  60208, USA}
\author{D.~J.~Ottaway}\affiliation{LIGO - Massachusetts Institute of Technology, Cambridge, MA
02139, USA}
\author{H.~Overmier}\affiliation{LIGO Livingston Observatory, Livingston, LA  70754, USA}
\author{B.~J.~Owen}\affiliation{The Pennsylvania State University, University Park, PA  16802, USA}
\author{Y.~Pan}\affiliation{University of Maryland, College Park, MD 20742 USA}
\author{M.~A.~Papa}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur
Gravitationsphysik, D-14476 Golm, Germany}\affiliation{University of Wisconsin-Milwaukee, Milwaukee,
WI  53201, USA}
\author{V.~Parameshwaraiah}\affiliation{LIGO Hanford Observatory, Richland, WA  99352, USA}
\author{C.~Parameswariah}\affiliation{LIGO Livingston Observatory, Livingston, LA  70754, USA}
\author{P.~Patel}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{M.~Pedraza}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{S.~Penn}\affiliation{Hobart and William Smith Colleges, Geneva, NY  14456, USA}
\author{V.~Pierro}\affiliation{University of Sannio at Benevento, I-82100 Benevento, Italy}
\author{I.~M.~Pinto}\affiliation{University of Sannio at Benevento, I-82100 Benevento, Italy}
\author{M.~Pitkin}\affiliation{University of Glasgow, Glasgow, G12 8QQ, United Kingdom}
\author{H.~Pletsch}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur
Gravitationsphysik, D-30167 Hannover, Germany}
\author{M.~V.~Plissi}\affiliation{University of Glasgow, Glasgow, G12 8QQ, United Kingdom}
\author{F.~Postiglione}\affiliation{University of Salerno, 84084 Fisciano (Salerno), Italy}
\author{R.~Prix}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur Gravitationsphysik,
D-14476 Golm, Germany}
\author{V.~Quetschke}\affiliation{University of Florida, Gainesville, FL  32611, USA}
\author{F.~Raab}\affiliation{LIGO Hanford Observatory, Richland, WA  99352, USA}
\author{D.~Rabeling}\affiliation{Australian National University, Canberra, 0200, Australia}
\author{H.~Radkins}\affiliation{LIGO Hanford Observatory, Richland, WA  99352, USA}
\author{R.~Rahkola}\affiliation{University of Oregon, Eugene, OR  97403, USA}
\author{N.~Rainer}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur
Gravitationsphysik, D-30167 Hannover, Germany}
\author{M.~Rakhmanov}\affiliation{The Pennsylvania State University, University Park, PA  16802,
USA}
\author{K.~Rawlins}\affiliation{LIGO - Massachusetts Institute of Technology, Cambridge, MA 02139,
USA}
\author{S.~Ray-Majumder}\affiliation{University of Wisconsin-Milwaukee, Milwaukee, WI  53201, USA}
\author{V.~Re}\affiliation{University of Birmingham, Birmingham, B15 2TT, United Kingdom}
\author{T.~Regimbau}\affiliation{Cardiff University, Cardiff, CF2 3YB, United Kingdom}
\author{H.~Rehbein}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur
Gravitationsphysik, D-30167 Hannover, Germany}
\author{S.~Reid}\affiliation{University of Glasgow, Glasgow, G12 8QQ, United Kingdom}
\author{D.~H.~Reitze}\affiliation{University of Florida, Gainesville, FL  32611, USA}
\author{L.~Ribichini}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur
Gravitationsphysik, D-30167 Hannover, Germany}
\author{R.~Riesen}\affiliation{LIGO Livingston Observatory, Livingston, LA  70754, USA}
\author{K.~Riles}\affiliation{University of Michigan, Ann Arbor, MI  48109, USA}
\author{B.~Rivera}\affiliation{LIGO Hanford Observatory, Richland, WA  99352, USA}
\author{N.~A.~Robertson}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125,
USA}\affiliation{University of Glasgow, Glasgow, G12 8QQ, United Kingdom}
\author{C.~Robinson}\affiliation{Cardiff University, Cardiff, CF2 3YB, United Kingdom}
\author{E.~L.~Robinson}\affiliation{University of Birmingham, Birmingham, B15 2TT, United Kingdom}
\author{S.~Roddy}\affiliation{LIGO Livingston Observatory, Livingston, LA  70754, USA}
\author{A.~Rodriguez}\affiliation{Louisiana State University, Baton Rouge, LA  70803, USA}
\author{A.~M.~Rogan}\affiliation{Washington State University, Pullman, WA 99164, USA}
\author{J.~Rollins}\affiliation{Columbia University, New York, NY  10027, USA}
\author{J.~D.~Romano}\affiliation{Cardiff University, Cardiff, CF2 3YB, United Kingdom}
\author{J.~Romie}\affiliation{LIGO Livingston Observatory, Livingston, LA  70754, USA}
\author{R.~Route}\affiliation{Stanford University, Stanford, CA  94305, USA}
\author{S.~Rowan}\affiliation{University of Glasgow, Glasgow, G12 8QQ, United Kingdom}
\author{A.~R\"udiger}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur
Gravitationsphysik, D-30167 Hannover, Germany}
\author{L.~Ruet}\affiliation{LIGO - Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{P.~Russell}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{K.~Ryan}\affiliation{LIGO Hanford Observatory, Richland, WA  99352, USA}
\author{S.~Sakata}\affiliation{National Astronomical Observatory of Japan, Tokyo  181-8588, Japan}
\author{M.~Samidi}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{L.~Sancho~de~la~Jordana}\affiliation{Universitat de les Illes Balears, E-07122 Palma de
Mallorca, Spain}
\author{V.~Sandberg}\affiliation{LIGO Hanford Observatory, Richland, WA  99352, USA}
\author{G.~H.~Sanders}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125,
USA}
\author{V.~Sannibale}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125,
USA}
\author{S.~Saraf}\affiliation{Rochester Institute of Technology, Rochester, NY 14623, USA}
\author{P.~Sarin}\affiliation{LIGO - Massachusetts Institute of Technology, Cambridge, MA 02139,
USA}
\author{B.~S.~Sathyaprakash}\affiliation{Cardiff University, Cardiff, CF2 3YB, United Kingdom}
\author{S.~Sato}\affiliation{National Astronomical Observatory of Japan, Tokyo  181-8588, Japan}
\author{P.~R.~Saulson}\affiliation{Syracuse University, Syracuse, NY  13244, USA}
\author{R.~Savage}\affiliation{LIGO Hanford Observatory, Richland, WA  99352, USA}
\author{P.~Savov}\affiliation{Caltech-CaRT, Pasadena, CA  91125, USA}
\author{A.~Sazonov}\affiliation{University of Florida, Gainesville, FL  32611, USA}
\author{S.~Schediwy}\affiliation{University of Western Australia, Crawley, WA 6009, Australia}
\author{R.~Schilling}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur
Gravitationsphysik, D-30167 Hannover, Germany}
\author{R.~Schnabel}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur
Gravitationsphysik, D-30167 Hannover, Germany}
\author{R.~Schofield}\affiliation{University of Oregon, Eugene, OR  97403, USA}
\author{B.~F.~Schutz}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur
Gravitationsphysik, D-14476 Golm, Germany}\affiliation{Cardiff University, Cardiff, CF2 3YB, United
Kingdom}
\author{P.~Schwinberg}\affiliation{LIGO Hanford Observatory, Richland, WA  99352, USA}
\author{S.~M.~Scott}\affiliation{Australian National University, Canberra, 0200, Australia}
\author{A.~C.~Searle}\affiliation{Australian National University, Canberra, 0200, Australia}
\author{B.~Sears}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{F.~Seifert}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur
Gravitationsphysik, D-30167 Hannover, Germany}
\author{D.~Sellers}\affiliation{LIGO Livingston Observatory, Livingston, LA  70754, USA}
\author{A.~S.~Sengupta}\affiliation{Cardiff University, Cardiff, CF2 3YB, United Kingdom}
\author{P.~Shawhan}\affiliation{University of Maryland, College Park, MD 20742 USA}
\author{D.~H.~Shoemaker}\affiliation{LIGO - Massachusetts Institute of Technology, Cambridge, MA
02139, USA}
\author{A.~Sibley}\affiliation{LIGO Livingston Observatory, Livingston, LA  70754, USA}
\author{J.~A.~Sidles}\affiliation{University of Washington, Seattle, WA, 98195}
\author{X.~Siemens}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125,
USA}\affiliation{Caltech-CaRT, Pasadena, CA  91125, USA}
\author{D.~Sigg}\affiliation{LIGO Hanford Observatory, Richland, WA  99352, USA}
\author{S.~Sinha}\affiliation{Stanford University, Stanford, CA  94305, USA}
\author{A.~M.~Sintes}\affiliation{Universitat de les Illes Balears, E-07122 Palma de Mallorca,
Spain}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur Gravitationsphysik, D-14476
Golm, Germany}
\author{B.~J.~J.~Slagmolen}\affiliation{Australian National University, Canberra, 0200, Australia}
\author{J.~Slutsky}\affiliation{Louisiana State University, Baton Rouge, LA  70803, USA}
\author{J.~R.~Smith}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur
Gravitationsphysik, D-30167 Hannover, Germany}
\author{M.~R.~Smith}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125,
USA}
\author{K.~Somiya}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur
Gravitationsphysik, D-30167 Hannover, Germany}\affiliation{Albert-Einstein-Institut,
Max-Planck-Institut f\"ur Gravitationsphysik, D-14476 Golm, Germany}
\author{K.~A.~Strain}\affiliation{University of Glasgow, Glasgow, G12 8QQ, United Kingdom}
\author{D.~M.~Strom}\affiliation{University of Oregon, Eugene, OR  97403, USA}
\author{A.~Stuver}\affiliation{The Pennsylvania State University, University Park, PA  16802, USA}
\author{T.~Z.~Summerscales}\affiliation{Andrews University, Berrien Springs, MI 49104 USA}
\author{K.-X.~Sun}\affiliation{Stanford University, Stanford, CA  94305, USA}
\author{M.~Sung}\affiliation{Louisiana State University, Baton Rouge, LA  70803, USA}
\author{P.~J.~Sutton}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125,
USA}
\author{H.~Takahashi}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur
Gravitationsphysik, D-14476 Golm, Germany}
\author{D.~B.~Tanner}\affiliation{University of Florida, Gainesville, FL  32611, USA}
\author{M.~Tarallo}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{R.~Taylor}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{R.~Taylor}\affiliation{University of Glasgow, Glasgow, G12 8QQ, United Kingdom}
\author{J.~Thacker}\affiliation{LIGO Livingston Observatory, Livingston, LA  70754, USA}
\author{K.~A.~Thorne}\affiliation{The Pennsylvania State University, University Park, PA  16802,
USA}
\author{K.~S.~Thorne}\affiliation{Caltech-CaRT, Pasadena, CA  91125, USA}
\author{A.~Th\"uring}\affiliation{Universit\"at Hannover, D-30167 Hannover, Germany}
\author{K.~V.~Tokmakov}\affiliation{University of Glasgow, Glasgow, G12 8QQ, United Kingdom}
\author{C.~Torres}\affiliation{The University of Texas at Brownsville and Texas Southmost College,
Brownsville, TX  78520, USA}
\author{C.~Torrie}\affiliation{University of Glasgow, Glasgow, G12 8QQ, United Kingdom}
\author{G.~Traylor}\affiliation{LIGO Livingston Observatory, Livingston, LA  70754, USA}
\author{M.~Trias}\affiliation{Universitat de les Illes Balears, E-07122 Palma de Mallorca, Spain}
\author{W.~Tyler}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{D.~Ugolini}\affiliation{Trinity University, San Antonio, TX  78212, USA}
\author{C.~Ungarelli}\affiliation{University of Birmingham, Birmingham, B15 2TT, United Kingdom}
\author{K.~Urbanek}\affiliation{Stanford University, Stanford, CA  94305, USA}
\author{H.~Vahlbruch}\affiliation{Universit\"at Hannover, D-30167 Hannover, Germany}
\author{M.~Vallisneri}\affiliation{Caltech-CaRT, Pasadena, CA  91125, USA}
\author{C.~Van~Den~Broeck}\affiliation{Cardiff University, Cardiff, CF2 3YB, United Kingdom}
\author{M.~van~Putten}\affiliation{LIGO - Massachusetts Institute of Technology, Cambridge, MA
02139, USA}
\author{M.~Varvella}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125,
USA}
\author{S.~Vass}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{A.~Vecchio}\affiliation{University of Birmingham, Birmingham, B15 2TT, United Kingdom}
\author{J.~Veitch}\affiliation{University of Glasgow, Glasgow, G12 8QQ, United Kingdom}
\author{P.~Veitch}\affiliation{University of Adelaide, Adelaide, SA 5005, Australia}
\author{A.~Villar}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{C.~Vorvick}\affiliation{LIGO Hanford Observatory, Richland, WA  99352, USA}
\author{S.~P.~Vyachanin}\affiliation{Moscow State University, Moscow, 119992, Russia}
\author{S.~J.~Waldman}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125,
USA}
\author{L.~Wallace}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{H.~Ward}\affiliation{University of Glasgow, Glasgow, G12 8QQ, United Kingdom}
\author{R.~Ward}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{K.~Watts}\affiliation{LIGO Livingston Observatory, Livingston, LA  70754, USA}
\author{D.~Webber}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{A.~Weidner}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur
Gravitationsphysik, D-30167 Hannover, Germany}
\author{M.~Weinert}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur
Gravitationsphysik, D-30167 Hannover, Germany}
\author{A.~Weinstein}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125,
USA}
\author{R.~Weiss}\affiliation{LIGO - Massachusetts Institute of Technology, Cambridge, MA 02139,
USA}
\author{S.~Wen}\affiliation{Louisiana State University, Baton Rouge, LA  70803, USA}
\author{K.~Wette}\affiliation{Australian National University, Canberra, 0200, Australia}
\author{J.~T.~Whelan}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur
Gravitationsphysik, D-14476 Golm, Germany}
\author{D.~M.~Whitbeck}\affiliation{The Pennsylvania State University, University Park, PA  16802,
USA}
\author{S.~E.~Whitcomb}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125,
USA}
\author{B.~F.~Whiting}\affiliation{University of Florida, Gainesville, FL  32611, USA}
\author{S.~Wiley}\affiliation{California State University Dominguez Hills, Carson, CA  90747, USA}
\author{C.~Wilkinson}\affiliation{LIGO Hanford Observatory, Richland, WA  99352, USA}
\author{P.~A.~Willems}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125,
USA}
\author{L.~Williams}\affiliation{University of Florida, Gainesville, FL  32611, USA}
\author{B.~Willke}\affiliation{Universit\"at Hannover, D-30167 Hannover,
Germany}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur Gravitationsphysik, D-30167
Hannover, Germany}
\author{I.~Wilmut}\affiliation{Rutherford Appleton Laboratory, Chilton, Didcot, Oxon OX11 0QX United
Kingdom}
\author{W.~Winkler}\affiliation{Albert-Einstein-Institut, Max-Planck-Institut f\"ur
Gravitationsphysik, D-30167 Hannover, Germany}
\author{C.~C.~Wipf}\affiliation{LIGO - Massachusetts Institute of Technology, Cambridge, MA 02139,
USA}
\author{S.~Wise}\affiliation{University of Florida, Gainesville, FL  32611, USA}
\author{A.~G.~Wiseman}\affiliation{University of Wisconsin-Milwaukee, Milwaukee, WI  53201, USA}
\author{G.~Woan}\affiliation{University of Glasgow, Glasgow, G12 8QQ, United Kingdom}
\author{D.~Woods}\affiliation{University of Wisconsin-Milwaukee, Milwaukee, WI  53201, USA}
\author{R.~Wooley}\affiliation{LIGO Livingston Observatory, Livingston, LA  70754, USA}
\author{J.~Worden}\affiliation{LIGO Hanford Observatory, Richland, WA  99352, USA}
\author{W.~Wu}\affiliation{University of Florida, Gainesville, FL  32611, USA}
\author{I.~Yakushin}\affiliation{LIGO Livingston Observatory, Livingston, LA  70754, USA}
\author{H.~Yamamoto}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125,
USA}
\author{Z.~Yan}\affiliation{University of Western Australia, Crawley, WA 6009, Australia}
\author{S.~Yoshida}\affiliation{Southeastern Louisiana University, Hammond, LA  70402, USA}
\author{N.~Yunes}\affiliation{The Pennsylvania State University, University Park, PA  16802, USA}
\author{M.~Zanolin}\affiliation{LIGO - Massachusetts Institute of Technology, Cambridge, MA 02139,
USA}
\author{J.~Zhang}\affiliation{University of Michigan, Ann Arbor, MI  48109, USA}
\author{L.~Zhang}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\author{C.~Zhao}\affiliation{University of Western Australia, Crawley, WA 6009, Australia}
\author{N.~Zotov}\affiliation{Louisiana Tech University, Ruston, LA  71272, USA}
\author{M.~Zucker}\affiliation{LIGO - Massachusetts Institute of Technology, Cambridge, MA 02139,
USA}
\author{H.~zur~M\"uhlen}\affiliation{Universit\"at Hannover, D-30167 Hannover, Germany}
\author{J.~Zweizig}\affiliation{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\collaboration{The LIGO Scientific Collaboration, http://www.ligo.org}
\noaffiliation
\author{M.~Kramer}\affiliation{University of Manchester, Jodrell Bank Observatory, Macclesfield,
SK11 9DL, United Kingdom}
\author{A.~G.~Lyne}\affiliation{University of Manchester, Jodrell Bank Observatory, Macclesfield,
SK11 9DL, United Kingdom}


